Guided Depth Super-Resolution by Deep Anisotropic Diffusion

Performing super-resolution of a depth image using the guidance from an RGB image is a problem that concerns several fields, such as robotics, medical imaging, and remote sensing. While deep learning methods have achieved good results in this problem, recent work highlighted the value of combining modern methods with more formal frameworks. In this work, we propose a novel approach which combines guided anisotropic diffusion with a deep convolutional network and advances the state of the art for guided depth super-resolution. The edge transferring/enhancing properties of the diffusion are boosted by the contextual reasoning capabilities of modern networks, and a strict adjustment step guarantees perfect adherence to the source image. We achieve unprecedented results in three commonly used benchmarks for guided depth super-resolution. The performance gain compared to other methods is the largest at larger scales, such as x32 scaling. Code (https://github.com/prs-eth/Diffusion-Super-Resolution) for the proposed method is available to promote reproducibility of our results.

==> diff_results.tex <==

%\newcommand\FigsGridWidth{0.106}
\newcommand\FigsGridWidth{0.09}
\newcommand\FigsGridVspace{0.05cm}
\newcommand\FigsGridVspacee{0.15cm}
\newcommand\FigsGridHspace{-0.22cm}
\newcommand\FigsGridHspacee{0.22cm}

\newcommand\MID{6}
\newcommand\MIDbis{400}

\newcommand\NYUv{5}
\newcommand\NYUvbis{103}

\newcommand\DIMLv{326}
\newcommand\DIMLvbis{4856}


\begin{figure*}[t]
\vspace{-0.2cm}
  \centering
  \tiny	
% \begin{center}
% 	\hspace{1.5cm}\includegraphics[width=0.25\linewidth]{diffs/colorbar}\vspace{-.5cm}
% \end{center}

%0.141 0.106
\subfloat[{Guide.}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
        
        \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/guide_\MID.png}\vspace{\FigsGridVspace} 
        \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/guide_\MIDbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
        \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/guide_\NYUv.png}\vspace{\FigsGridVspace}
        \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/guide_\NYUvbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/guide_\DIMLv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/guide_\DIMLvbis.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{Source}.]{

    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/source_idx_\MID_scale_8.png}\vspace{\FigsGridVspace} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/source_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/source_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/source_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/source_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/source_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}

}\hspace{\FigsGridHspace}
\subfloat[{GT}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/gt_idx_\MID.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/gt_idx_\MIDbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/gt_idx_\NYUv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/gt_idx_\NYUvbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/gt_idx_\DIMLv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/gt_idx_\DIMLvbis.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{SD}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/SDfilter_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/SDfilter_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/SDfilter_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/SDfilter_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/SDfilter_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/SDfilter_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{Pixtr}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/pixtransform_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/pixtransform_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}  
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/pixtransform_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/pixtransform_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/pixtransform_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/pixtransform_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{MSG}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/MSGNet_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/MSGNet_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/MSGNet_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/MSGNet_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/MSGNet_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/MSGNet_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{FDKN}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/fdkn_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/fdkn_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/fdkn_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/fdkn_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/fdkn_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/fdkn_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{PMBA}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/pmba_full_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/pmba_full_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/pmba_full_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/pmba_full_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/pmba_full_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/pmba_full_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{FDSR}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/FDSR_theirs_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/FDSR_theirs_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/FDSR_theirs_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/FDSR_theirs_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/FDSR_theirs_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/FDSR_theirs_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{Ours}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/ours_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/ours_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/ours_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/ours_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/ours_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/ours_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{Ours Pred}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/ours_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/ours_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/ours_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/ours_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/ours_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/ours_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}
\caption{Qualitative comparison of upsampled depth maps. From top to bottom each group of two rows shows the error of upsampled images, defined as the difference between the prediction and the ground truth, on the Middlebury \cite{Scharstein2007,Scharstein2001,Scharstein2014,Scharstein2003,Hirschmuller2007}, NYUv2 \cite{Silberman2012} and DIML \cite{DIML1,DIML2,DIML3,DIML4} datasets, respectively; alternating between upsampling factors $\times8$ and $\times16$ for each dataset. From left to right, the first group of columns are (a) Guide, (b) Source and (c) Ground Truth; the second group includes selected methods from our quantitative evaluation, (d) SD filter \cite{Ham2018}, (e) Pixtransform \cite{deLutio2019}, (f) MSG-Net \cite{Tak-Wai2016}, (g) FDKN \cite{Kim2021}, (h) PMBANet \cite{Ye2020} and (i) FDSR \cite{he2021}; the last two columns represent (j) the error for the prediction of our model and (k) the prediction itself.}
\label{fig:depth_upsampling}
\vspace{-0.3cm}
\end{figure*}

==> tables/additional_metrics.tex <==
\begin{table}[h]
\centering
\footnotesize
 % \resizebox{0.475\textwidth}{!}{%
\begin{tabularx}{0.40\textwidth}{l| YYY}
 & \multicolumn{3}{c}{Middlebury} & \multicolumn{3}{c}{NYUv2} \midrule \\
 [\%] & V-err & E-err & MAPE \\ \midrule 
 MSG          & ? & ? & ?  \\
 DKN          & ? & ? & ?  \\
 FDKN         & ? & ? & ?  \\
 PMBA         & ? & ? & ?  \\
 FDSR         & ? & ? & ?  \\
 LGR          & ? & ? & ?  \\
 DADA         & ? & ? & ?
\end{tabularx}%
 % }%\usepackage{adjustbox}
\caption{}
\label{tab:encoders}
\end{table}



==> tables/additional_metrics_v2.tex <==
\begin{table}[h]
\centering
\footnotesize
\vspace{-0.075cm}
 \resizebox{0.45\textwidth}{!}{%
\begin{tabular}{l| ccc}
 \multicolumn{1}{c}{} & \textbf{Middlebury} & \textbf{NYUv2} & \textbf{DIML}  \\ 
 \multicolumn{1}{c}{in $[\%]$} &       MAPE/VE/EE & MAPE/VE/EE & MAPE/VE/EE  \\ \midrule  
 MSG          &  0.8 / 1.7 / 14.7 &  1.9 / 3.0 / 49.8 &  0.9 / 1.2 / 24.8 \\
 DKN          &  1.2 / 2.7 / 21.9 &  2.4 / 4.4 / 55.8 &  1.4 / 2.2 / 32.3 \\
 FDKN         &  1.2 / 2.6 / 21.7 &  2.4 / 4.5 / 55.7 &  1.4 / 2.2 / 34.3 \\
 PMBA         &  1.9 / 4.1 / 35.7 &  2.7 / 5.2 / 57.4 &  0.8 / 1.2 / 25.0 \\
 FDSR         &  1.6 / 3.7 / 21.6 &  3.4 / 7.2 / 63.4 &  1.6 / 2.5 / 36.3 \\
 LGR          &  0.6 / 1.2 / 12.8 &  1.8 / 2.7 / 49.0 &  0.9 / 1.3 / 26.7 \\
 DADA         &  \textbf{0.5} / \textbf{0.9} / \textbf{8.1} &  \textbf{1.6} / \textbf{2.4} / \textbf{44.3} &  \textbf{0.7} / \textbf{0.9} / \textbf{19.7}
\end{tabular}%
 }%\usepackage{adjustbox}
 \vspace{-0.1cm}
\caption{Middlebury, scale x32, all numbers are in [\%].}
\vspace{-0.2cm}
\label{tab:new_metrics}
\end{table}


==> tables/encoders.tex <==
\begin{table}[h]
\centering
\footnotesize
 \resizebox{0.475\textwidth}{!}{%
\begin{tabular}{l| c | ccccccc}
 \multicolumn{1}{c}{} & U-Net & U-Net & U-Net & U-Net & U-Net & U-Net & FPN  & DL3+  \\ 
 \multicolumn{1}{c}{}  & RN50 & RN34  & RN18  & ENB2 & ENB1 & ENB0  & RN50 & RN50  \\  \midrule 
  % \#layers & & & & & & & \\ \midrule  
 MSE          & 5.60  & 5.57 & 5.69  & 6.68 & 6.77 & 6.85 & 7.09 & 7.77 \\
 MAE          & 0.20  & 0.20 & 0.20  & 0.24 & 0.24 & 0.24 & 0.27 & 0.30 \\
 
\end{tabular}%
 }%\usepackage{adjustbox}
\vspace{-0.1cm}
\caption{DADA is insensitive to the depth of the feature extractor.}
\vspace{-0.1cm}
\label{tab:encoders}
\end{table}

==> tables/encoders_v2.tex <==
\begin{table}[h]
\centering
\footnotesize
 \resizebox{0.475\textwidth}{!}{%
\begin{tabular}{l| cccccccc}
 \multicolumn{1}{c}{} & U-Net & U-Net & \textbf{U-Net} & U-Net & U-Net & U-Net & FPN  & DL3+  \\ 
 \multicolumn{1}{c}{}  & RN18 & RN34  & \textbf{RN50}  & ENB0 & ENB1 & ENB2  & RN50 & RN50  \\  \midrule 
  % \#layers & & & & & & & \\ \midrule  
 MSE          & 5.69  & 5.57 & 5.60  & 6.85 & 6.77 & 6.68 & 7.09 & 7.77 \\
 MAE          & 0.20  & 0.20 & 0.20  & 0.24 & 0.24 & 0.24 & 0.27 & 0.30 \\
 
\end{tabular}%
 }%\usepackage{adjustbox}
\vspace{-0.1cm}
\caption{Middlebury, scale x8. DADA is fairly insensitive to the depth of the feature extractor.}
\vspace{-0.1cm}
\label{tab:encoders}
\end{table}

==> tables/main_table_v1.tex <==

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l | cccccccc | cccccccc | cccccccc}
    % \toprule
     & \multicolumn{8}{c|}{Middlebury} & \multicolumn{8}{c|}{NYUv2} & \multicolumn{8}{c}{DIML} \\
     & \multicolumn{2}{c}{x4}  & \multicolumn{2}{c}{x8}  & \multicolumn{2}{c}{x16}  & \multicolumn{2}{c|}{x32} & \multicolumn{2}{c}{x4}  & \multicolumn{2}{c}{x8}  & \multicolumn{2}{c}{x16}  & \multicolumn{2}{c|}{x32} & \multicolumn{2}{c}{x4}  & \multicolumn{2}{c}{x8}  & \multicolumn{2}{c}{x16}  & \multicolumn{2}{c}{x32} \\
     & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\ \midrule \midrule
    GF & 33.3 & 1.27 & 40.5 & 1.49 & 67.4 & 2.21 &  &  & 114 & 3.91 & 142 & 4.47 & 249 & 6.34 &  &  & 25.6 & 1.45 & 34.1 & 1.77 & 66.3 & 2.74 &  & \\
    SD Filter & 24.9 &  0.46 & 82.5 & 0.86 & 511 & 1.73 &  &  & 36.0 & 1.31 & 105 &  2.57 & 533 & 5.07 &  &  & 10.5 &  0.40 &  44.9 & 0.83 & 411 &  1.91 &  & \\
    Pixtransform & 39.8 & 0.79 & 32.7 &  0.82 &  41.5 & \textbf{1.24} &  &  & 112 & 3.61 & 122 & 3.86 & 219 & 5.40 &  &  &  20.7 &  1.15 & 23.0 &  1.26 & 39.3 & 1.78 &  & \\
    Graph (color) & 14.8 &  0.42 & 68.3 & 0.83 & 297 & 1.69 &  &  &  19.0 & 1.11 &  68.4 & 2.30 & 264 & 4.56 &  &  &  7.02 & 0.35 & 15.2 & 0.67 & 133 & 1.72 &  & \\
    Ours (color)    & \textbf{11.1} & \textbf{0.40} & \textbf{18.9} & \textbf{0.70} & \textbf{36.7} & 1.30 & \textbf{83.5} & \textbf{2.59} & \textbf{18.1} & \textbf{1.05} & \textbf{49.9} & \textbf{2.05} & \textbf{125} & \textbf{3.88} & \textbf{336} & \textbf{7.64} & \textbf{4.40} & \textbf{0.28} & \textbf{9.35} & \textbf{0.51} & \textbf{21.3} & \textbf{1.15} & \textbf{73.1} & \textbf{3.05} \\ \midrule
    % Ours (color, learned K) & \textbf{11.1} & \textbf{0.40} & \textbf{18.4} & \textbf{0.68} & \textbf{35.5} & 1.25 & \textbf{82.8} & \textbf{2.56} & \textbf{14.8} & \textbf{1.03} & \textbf{45.9} & \textbf{2.04} & \textbf{125} & 3.89 & \textbf{330} & \textbf{7.59} & \textbf{4.05} & \textbf{0.27} & \textbf{9.09} & \textbf{0.51} & 21.4 & \textbf{1.15} & \textbf{73.1} & \textbf{3.05} \\ \midrule
    MSG-Net & 4.13 & 0.22 & 10.5 & 0.43 & 34.2 &  1.06 &  &  & 6.85 &  0.81 & 24.1 & 1.66 &  84.5 & 3.35 &  &  &  1.73 & 0.22 & 4.13 &  0.40 &  13.0 & 0.93 &  & \\
    DKN & 4.29 & 0.18 & 11.2 &  0.38 & 47.6 &  1.42 &  &  &  11.4 & 1.03 &  29.8 & 1.82 & 115 & 4.01 &  &  & 3.47 &  0.33 &  5.47 & 0.45 & 19.3 & 1.20 &  & \\
    FDKN & 3.60 & 0.16 & 10.4 &  0.37 &  38.5 & 1.18 &  &  & 8.07 & 0.85 &  29.9 &  1.80 & 113 & 3.95 &  &  &  2.2 &  0.23 & 5.95 & 0.47 & 20.8 & 1.24 &  & \\
    PMBANet & 4.72 & 0.25 &  9.48 & 0.38 & 30.6 &  0.89 &  &  & 10.8 &  0.93 & 31.5 & 1.79 &  84.9 &  3.26 &  &  & 3.05 &  0.31 &  5.87 & 0.47 & 13.8 & 0.87 &  & \\
    FDSR & 7.72 & 0.35 & 23.2 & 0.69 & 55.4 & 1.51 &  &  &  10.5 & 0.94 & 35.4 &  1.96 & 179 & 4.68 &  &  & 2.75 & 0.29 & 8.40 & 0.66 & 32.9 &  1.66 &  & \\
    Graph (learned) & 3.04 & 0.13 & 7.26 & 0.24 & 24.7 & 0.67 &  &  & 6.45 & 0.73 & 19.6 & 1.42 & 67.5 & 2.90 &  &  & 1.68 & 0.20 & 3.51 & 0.31 & 9.45 & 0.68 &  & \\
    Ours (learned) & \textbf{2.55} & \textbf{0.11} & \textbf{5.81} & \textbf{0.21} & \textbf{14.9} & \textbf{0.47} & \textbf{50.0} & \textbf{1.40} & \textbf{4.98} & \textbf{0.64} & \textbf{17.1} & \textbf{1.31} & \textbf{57.1} & \textbf{2.60} & \textbf{216} & \textbf{5.67} & \textbf{1.36} & \textbf{0.17} & \textbf{2.89} & \textbf{0.27} & \textbf{7.58} & \textbf{0.58} & \textbf{36.3} & \textbf{1.83} \\ %\bottomrule
    
    \end{tabular}%
    }
    \caption{Performance comparison.}
    \label{tab:cmp}
\end{table*}


==> tables/main_table_v2.tex <==

\begin{table*}[t]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{ll | cccccc | cccccc | cccccc}
    % \toprule
     &  & \multicolumn{6}{c|}{\textbf{Middlebury}} & \multicolumn{6}{c|}{\textbf{NYUv2}} & \multicolumn{6}{c}{\textbf{DIML}} \\
     &  & \multicolumn{2}{c}{x4}  & \multicolumn{2}{c}{x8}  & \multicolumn{2}{c|}{x16} & \multicolumn{2}{c}{x4}  & \multicolumn{2}{c}{x8}  & \multicolumn{2}{c|}{x16}  & \multicolumn{2}{c}{x4}  & \multicolumn{2}{c}{x8}  & \multicolumn{2}{c}{x16} \\
     &  & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\ \midrule \midrule
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Heuristic}}}} & Bicubic & 13.3 & 0.55 & 30.0 & 1.10 & 68.5  & 2.13 & 31.87 & 1.59  & 89.9  &  3.17  & 242 & 6.01 & 10.4 & 0.63 & 28.555 & 1.315  &  73.23 &  2.68  \\
     & GF & 33.3 & 1.27 & 40.5 & 1.49 & 67.4 & 2.21 & 114 & 3.91 & 142 & 4.47 & 249 & 6.34 & 25.6 & 1.45 & 34.1 & 1.77 & 66.3 & 2.74 \\
     & SD Filter & 24.9 (46.7) &  0.46 (0.695) & 82.5 & 0.86 & 511 (135.93) & 1.73 (2.73) & 36.0 & 1.31 & 105 &  2.57 & 533 & 5.07 & 10.5 &  0.40 &  44.9 & 0.83 & 411 &  1.91 \\
     & SD Filter & 24.9 &  0.46 & 82.5 & 0.86 & 511 & 1.73 & 36.0 & 1.31 & 105 &  2.57 & 533 & 5.07 & 10.5 &  0.40 &  44.9 & 0.83 & 411 &  1.91 \\
     & Pixtransform & 39.8 & 0.79 & 32.7 & 0.82 &  41.5 & \textbf{1.24} & 112 & 3.61 & 122 & 3.86 & 219 & 5.40 & 20.7 &  1.15 & 23.0 &  1.26 & 39.3 & 1.78 \\
     & Graph (color) & 14.8 &  0.42 & 68.3 & 0.83 & 297 & 1.69 &  19.0 & 1.11 &  68.4 & 2.30 & 264 & 4.56 & 7.02 & 0.35 & 15.2 & 0.67 & 133 & 1.72 \\
     & Ours (color)    & \textbf{11.1} & \textbf{0.40} & \textbf{18.9} & \textbf{0.70} & \textbf{36.7} & 1.30 & \textbf{18.1} & \textbf{1.05} & \textbf{49.9} & \textbf{2.05} & \textbf{125} & \textbf{3.88} & \textbf{4.40} & \textbf{0.28} & \textbf{9.35} & \textbf{0.51} & \textbf{21.3} & \textbf{1.15} \\ \midrule
    \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Learned}}}} & MSG-Net & 4.13 & 0.22 & 10.5 & 0.43 & 34.2 &  1.06 & 6.85 & 0.81 & 24.1 & 1.66 &  84.5 & 3.35 & 1.73 & 0.22 & 4.13 &  0.40 &  13.0 & 0.93 \\
     & DKN & 4.29 & 0.18 & 11.2 &  0.38 & 47.6 &  1.42 & 11.4 & 1.03 &  29.8 & 1.82 & 115 & 4.01 & 3.47 &  0.33 &  5.47 & 0.45 & 19.3 & 1.20 \\
     & FDKN & 3.60 & 0.16 & 10.4 &  0.37 &  38.5 & 1.18 & 8.07 & 0.85 &  29.9 &  1.80 & 113 & 3.95 & 2.2 & 0.23 & 5.95 & 0.47 & 20.8 & 1.24 \\
     & PMBANet & 4.72 & 0.25 &  9.48 & 0.38 & 30.6 &  0.89 & 10.8 &  0.93 & 31.5 & 1.79 &  84.9 &  3.26 & 3.05 &  0.31 &  5.87 & 0.47 & 13.8 & 0.87 \\
     & FDSR & 7.72 & 0.35 & 23.2 & 0.69 & 55.4 & 1.51 & 10.5 & 0.94 & 35.4 &  1.96 & 179 & 4.68 & 2.75 & 0.29 & 8.40 & 0.66 & 32.9 &  1.66 \\
     & Graph (learned) & 3.04 & 0.13 & 7.26 & 0.24 & 24.7 & 0.67 & 6.45 & 0.73 & 19.6 & 1.42 & 67.5 & 2.90 & 1.68 & 0.20 & 3.51 & 0.31 & 9.45 & 0.68 \\
    %  & Ours (learned) & \textbf{2.55} & \textbf{0.11} & \textbf{5.81} & \textbf{0.21} & \textbf{14.9} & \textbf{0.47} & \textbf{4.98} & \textbf{0.64} & \textbf{17.1} & \textbf{1.31} & \textbf{57.1} & \textbf{2.60} & \textbf{1.36} & \textbf{0.17} & \textbf{2.89} & \textbf{0.27} & \textbf{7.58} & \textbf{0.58} \\ %\bottomrule
     & Ours (learned) & \textbf{2.50} & \textbf{0.10} & \textbf{5.67} & \textbf{0.20} & \textbf{16.3} & \textbf{0.48} & \textbf{4.83} & \textbf{0.64} & \textbf{16.8} & \textbf{1.32} & \textbf{59.0} & \textbf{2.64} & \textbf{1.33} & \textbf{0.17} & \textbf{2.93} & \textbf{0.28} & \textbf{7.61} & \textbf{0.59} \\ %\bottomrule
    \end{tabular}%
    }
    \caption{Performance comparison.}
    \label{tab:cmp}
\end{table*}


==> tables/main_table_v3.tex <==

\begin{table}[t]
    \centering
    \resizebox{0.475\textwidth}{!}{%
    \begin{tabular}{ll | cc|cc|cc|cc}
    % \toprule
     &  & \multicolumn{2}{c|}{x4}  & \multicolumn{2}{c|}{x8}  & \multicolumn{2}{c|}{x16}  & \multicolumn{2}{c}{x32}  \\
     &  & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE  \\ \midrule \midrule
     &  & \multicolumn{8}{c}{\textbf{Middlebury}}  \\ \midrule
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-free}}}} & Bicubic & 13.3 & 0.55 & 30.0 & 1.10 & 68.5  & 2.13 & 143 & 3.87 \\
     & GF & 33.3 & 1.27 & 40.5 & 1.49 & 67.4 & 2.21 & 134 & 3.82  \\
     & SD Filter & 24.9 &  0.46 & 82.5 & 0.86 & 511 & 1.73 & 4062 & 3.37 \\
     & Pixtransform & 39.8 & 0.79 & 32.7 & 0.82 &  41.5 & \textbf{1.24} & 107 & 2.71 \\
     & LGR (color) & 14.8 &  0.42 & 68.3 & 0.83 & 297 & 1.69 & 897 & 3.31 \\
     & Ours (color)  & \textbf{11.1} & \textbf{0.40} & \textbf{18.9} & \textbf{0.70} & \textbf{36.7} & 1.30 & \textbf{84.1} & \textbf{2.58} \\ \midrule
    \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-based}}}} & MSG-Net & 4.13 & 0.22 & 10.5 & 0.43 & 34.2 & 1.06 & 92.9 & 2.55 \\
     & DKN & 4.29 & 0.18 & 11.2 &  0.38 & 47.6 &  1.42 & 119 & 3.35 \\
     & FDKN & 3.60 & 0.16 & 10.4 &  0.37 &  38.5 & 1.18 & 112 & 3.23 \\
     & PMBANet & 4.72 & 0.25 &  9.48 & 0.38 & 30.6 &  0.89 & 175 & 5.15 \\
     & FDSR & 7.72 & 0.35 & 23.2 & 0.69 & 55.4 & 1.51 &  179 & 4.11 \\
     & LGR & 3.04 & 0.13 & 7.26 & 0.24 & 24.7 & 0.67 & 63.4 & 1.75 \\
     & Ours & \textbf{2.58} & \textbf{0.11} & \textbf{5.68} & \textbf{0.20} & \textbf{16.3} & \textbf{0.48} & \textbf{50.6} & \textbf{1.38} \\ %\bottomrule

    \midrule \midrule 

     &  & \multicolumn{8}{c}{\textbf{NYUv2}}  \\ \midrule
    %  &  & \multicolumn{2}{c}{x4}  & \multicolumn{2}{c}{x8}  & \multicolumn{2}{c}{x16}  & \multicolumn{2}{c}{x32}  \\
    %  &  & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE  \\ \midrule \midrule
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-free}}}} & Bicubic &  31.9 & 1.59  & 89.9  &  3.17  & 242 & 6.01 & 588 & 10.5 \\
     & GF &  114 & 3.91 & 142 & 4.47 & 249 & 6.34 & 556 & 10.4 \\
     & SD Filter & 36.0 & 1.31 & 105 &  2.57 & 533 & 5.07 & 3246 & 10.4 \\
     & Pixtransform & 112 & 3.61 & 122 & 3.86 & 219 & 5.40 & 759 & 11.6 \\
     & LGR (color) &  19.0 & 1.11 &  68.4 & 2.30 & 264 & 4.56 & 790 & 9.31 \\
     & Ours (color)  & \textbf{18.1} & \textbf{1.05} & \textbf{49.9} & \textbf{2.05} & \textbf{125} & \textbf{3.88} & \textbf{328} & \textbf{7.50} \\ \midrule
    \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-based}}}} & MSG-Net & 6.85 & 0.81 & 24.1 & 1.66 &  84.5 & 3.35 & 262 & 6.70 \\
     & DKN & 11.4 & 1.03 &  29.8 & 1.82 & 115 & 4.01 & 364 & 8.33 \\
     & FDKN & 8.07 & 0.85 &  29.9 &  1.80 & 113 & 3.95 & 365 & 8.39 \\
     & PMBANet & 10.8 &  0.93 & 31.5 & 1.79 &  84.9 &  3.26 & 449 & 9.11 \\
     & FDSR & 10.5 & 0.94 & 35.4 &  1.96 & 179 & 4.68 &  771 & 11.8 \\
     & LGR & 6.45 & 0.73 & 19.6 & 1.42 & 67.5 & 2.90 & 253 & 6.50 \\
     & Ours & \textbf{4.83} & \textbf{0.64} & \textbf{16.6} & \textbf{1.30} & \textbf{59.0} & \textbf{2.64} & \textbf{228} & \textbf{5.81} \\ %\bottomrule

    \midrule \midrule 

     &  & \multicolumn{8}{c}{\textbf{DIML}}  \\ \midrule
    %  &  & \multicolumn{2}{c}{x4}  & \multicolumn{2}{c}{x8}  & \multicolumn{2}{c}{x16}  & \multicolumn{2}{c}{x32}  \\
    %  &  & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE  \\ \midrule \midrule
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-free}}}} & Bicubic & 10.4 & 0.63 & 28.6 & 1.32  &  73.2 &  2.68 & 187 & 5.37 \\
     & GF & 25.6 & 1.45 & 34.1 & 1.77 & 66.3 & 2.74 & 165 & 5.18 \\
     & SD Filter & 10.5 &  0.40 &  44.9 & 0.83 & 411 &  1.91 & -- & -- \\
     & Pixtransform &  20.7 &  1.15 & 23.0 &  1.26 & 39.3 & 1.78 & 141 & 4.19 \\
     & LGR (color) & 7.02 & 0.35 & 15.2 & 0.67 & 133 & 1.72 & 815 & 3.98 \\
     & Ours (color)  &  \textbf{4.40} & \textbf{0.28} & \textbf{9.35} & \textbf{0.51} & \textbf{21.3} & \textbf{1.15} & \textbf{72.6} & \textbf{3.02} \\ \midrule
    \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-based}}}} & MSG-Net & 1.73 & 0.22 & 4.13 &  0.40 &  13.0 & 0.93 & 55.0 & 2.56 \\
     & DKN & 3.47 &  0.33 &  5.47 & 0.45 & 19.3 & 1.20 & 91.5 & 3.75 \\
     & FDKN & 2.2 & 0.23 & 5.95 & 0.47 & 20.8 & 1.24 &  89.9 & 3.75 \\
     & PMBANet & 3.05 &  0.31 &  5.87 & 0.47 & 13.8 & 0.87 & 55.1 & 2.30 \\
     & FDSR & 2.75 & 0.29 & 8.40 & 0.66 & 32.9 &  1.66 & 124 & 4.39 \\
     & LGR & 1.68 & 0.20 & 3.51 & 0.31 & 9.45 & 0.68 & 57.0 & 2.47 \\
     & Ours & \textbf{1.33} & \textbf{0.17} & \textbf{2.93} & \textbf{0.28} & \textbf{7.61} & \textbf{0.59} & \textbf{39.8} & \textbf{1.92} \\ %\bottomrule
    \end{tabular}%
    }
    \caption{Performance comparison.}
    \label{tab:cmp}
\end{table}


==> tables/main_table_v4.tex <==

\begin{table}[t]
    \centering
    \resizebox{0.475\textwidth}{!}{%
    \begin{tabular}{ll | cccc}
    % \toprule
     &  & x4  & x8  & x16  & x32  \\
     &  & MSE/MAE & MSE/MAE & MSE/MAE & MSE/MAE  \\ \midrule \midrule
     &  & \multicolumn{4}{c}{\textbf{Middlebury}}  \\ \midrule
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-free}}}} & Bicubic & 13.3/0.55 & 30.0/1.10 & 68.5/2.13 & 143/3.87 \\
     & GF & 33.3/1.27 & 40.5/1.49 & 67.4/2.21 & 134/3.82  \\
     & SD & 24.9/0.46 & 82.5/0.86 & 511/1.73 & 4062/3.37 \\
     & PixT & 39.8/0.79 & 32.7/0.82 &  41.5/\textbf{1.24} & 107/2.71 \\
     & LGR$^\dag$ & 14.8/0.42 & 68.3/0.83 & 297/1.69 & 897/3.31 \\
     & Ours$^\dag$  & \textbf{11.1}/\textbf{0.40} & \textbf{18.9}/\textbf{0.70} & \textbf{36.7}/1.30 & \textbf{84.1}/\textbf{2.58} \\ \midrule
    \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-based}}}} & MSG & 4.13/0.22 & 10.5/0.43 & 34.2/1.06 & 92.9/2.55 \\
     & DKN & 4.29/0.18 & 11.2/0.38 & 47.6/1.42 & 119/3.35 \\
     & FDKN & 3.60/0.16 & 10.4/0.37 &  38.5/1.18 & 112/3.23 \\
     & PMBA & 4.72/0.25 & 9.48/0.38 & 30.6/0.89 & 175/5.15 \\
     & FDSR & 7.72/0.35 & 23.2/0.69 & 55.4/1.51 & 179/4.11 \\
     & LGR & 3.04/0.13 & 7.26/0.24 & 24.7/0.67 & 63.4/1.75 \\
     & Ours & \textbf{2.58}/\textbf{0.11} & \textbf{5.68}/\textbf{0.20} & \textbf{16.3}/\textbf{0.48} & \textbf{50.6}/\textbf{1.38} \\ %\bottomrule

    \midrule \midrule 

     &  & \multicolumn{4}{c}{\textbf{NYUv2}}  \\ \midrule
    %  &  & \multicolumn{2}{c}{x4}  & \multicolumn{2}{c}{x8}  & \multicolumn{2}{c}{x16}  & \multicolumn{2}{c}{x32}  \\
    %  &  & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE  \\ \midrule \midrule
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-free}}}} & Bicubic &  31.9/1.59  & 89.9/3.17  & 242/6.01 & 588/10.5 \\
     & GF &  114/3.91 & 142/4.47 & 249/6.34 & 556/10.4 \\
     & SD & 36.0/1.31 & 105/2.57 & 533/5.07 & 3246/10.4 \\
     & PixT & 112/3.61 & 122/3.86 & 219/5.40 & 759/11.6 \\
     & LGR$^\dag$ &  19.0/1.11 &  68.4/2.30 & 264/4.56 & 790/9.31 \\
     & Ours$^\dag$  & \textbf{18.1}/\textbf{1.05} & \textbf{49.9}/\textbf{2.05} & \textbf{125}/\textbf{3.88} & \textbf{328}/\textbf{7.50} \\ \midrule
    \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-based}}}} & MSG & 6.85/0.81 & 24.1/1.66 &  84.5/3.35 & 262/6.70 \\
     & DKN & 11.4/1.03 &  29.8/1.82 & 115/4.01 & 364/8.33 \\
     & FDKN & 8.07/0.85 &  29.9/1.80 & 113/3.95 & 365/8.39 \\
     & PMBA & 10.8/0.93 & 31.5/1.79 & 84.9/3.26 & 449/9.11 \\
     & FDSR & 10.5/0.94 & 35.4/1.96 & 179/4.68 & 771/11.8 \\
     & LGR & 6.45/0.73 & 19.6/1.42 & 67.5/2.90 & 253/6.50 \\
     & Ours & \textbf{4.83}/\textbf{0.64} & \textbf{16.6}/\textbf{1.30} & \textbf{59.0}/\textbf{2.64} & \textbf{228}/\textbf{5.81} \\ %\bottomrule

    \midrule \midrule 

     &  & \multicolumn{4}{c}{\textbf{DIML}}  \\ \midrule
    %  &  & \multicolumn{2}{c}{x4}  & \multicolumn{2}{c}{x8}  & \multicolumn{2}{c}{x16}  & \multicolumn{2}{c}{x32}  \\
    %  &  & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE  \\ \midrule \midrule
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-free}}}} & Bicubic & 10.4/0.63 & 28.6/1.32 & 73.2/2.68 & 187/5.37 \\
     & GF & 25.6/1.45 & 34.1/1.77 & 66.3/2.74 & 165/5.18 \\
     & SD & 10.5/0.40 & 44.9/0.83 & 411/1.91 & -- / -- \\
     & PixT &  20.7/1.15 & 23.0/1.26 & 39.3/1.78 & 141/4.19 \\
     & LGR$^\dag$ & 7.02/0.35 & 15.2/0.67 & 133/1.72 & 815/3.98 \\
     & Ours$^\dag$  &  \textbf{4.40}/\textbf{0.28} & \textbf{9.35}/\textbf{0.51} & \textbf{21.3}/\textbf{1.15} & \textbf{72.6}/\textbf{3.02} \\ \midrule
    \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Learning-based}}}} & MSG & 1.73/0.22 & 4.13/0.40 & 13.0/0.93 & 55.0/2.56 \\
     & DKN & 3.47/0.33 & 5.47/0.45 & 19.3/1.20 & 91.5/3.75 \\
     & FDKN & 2.2/0.23 & 5.95/0.47 & 20.8/1.24 & 89.9/3.75 \\
     & PMBA & 3.05/0.31 & 5.87/0.47 & 13.8/0.87 & 55.1/2.30 \\
     & FDSR & 2.75/0.29 & 8.40/0.66 & 32.9/1.66 & 124/4.39 \\
     & LGR & 1.68/0.20 & 3.51/0.31 & 9.45/0.68 & 57.0/2.47 \\
     & Ours & \textbf{1.33}/\textbf{0.17} & \textbf{2.93}/\textbf{0.28} & \textbf{7.61}/\textbf{0.59} & \textbf{39.8}/\textbf{1.92} \\ %\bottomrule
    \end{tabular}%
    }
    \caption{Performance comparison.}
    \label{tab:cmp}
\end{table}


==> tables/qualitative_results_v1.tex <==

%\newcommand\FigsGridWidth{0.106}
\newcommand\FigsGridWidth{0.09}
\newcommand\FigsGridVspace{0.05cm}
\newcommand\FigsGridVspacee{0.15cm}
\newcommand\FigsGridHspace{-0.22cm}
\newcommand\FigsGridHspacee{0.22cm}

\newcommand\MID{6}
\newcommand\MIDbis{400}

\newcommand\NYUv{5}
\newcommand\NYUvbis{103}

\newcommand\DIMLv{326}
\newcommand\DIMLvbis{4856}


\begin{figure*}[t]
\vspace{-0.2cm}
  \centering
  \tiny	
% \begin{center}
% 	\hspace{1.5cm}\includegraphics[width=0.25\linewidth]{diffs/colorbar}\vspace{-.5cm}
% \end{center}

%0.141 0.106
\subfloat[{Guide.}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
        
        \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/guide_\MID.png}\vspace{\FigsGridVspace} 
        \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/guide_\MIDbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
        \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/guide_\NYUv.png}\vspace{\FigsGridVspace}
        \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/guide_\NYUvbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/guide_\DIMLv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/guide_\DIMLvbis.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{Source}.]{

    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/source_idx_\MID_scale_8.png}\vspace{\FigsGridVspace} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/source_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/source_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/source_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/source_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/source_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}

}\hspace{\FigsGridHspace}
\subfloat[{GT}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/gt_idx_\MID.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/gt_idx_\MIDbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/gt_idx_\NYUv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/gt_idx_\NYUvbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/gt_idx_\DIMLv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/gt_idx_\DIMLvbis.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{SD}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/SDfilter_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/SDfilter_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/SDfilter_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/SDfilter_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/SDfilter_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/SDfilter_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{Pixtr}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/pixtransform_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/pixtransform_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}  
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/pixtransform_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/pixtransform_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/pixtransform_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/pixtransform_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{MSG}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/MSGNet_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/MSGNet_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/MSGNet_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/MSGNet_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/MSGNet_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/MSGNet_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{FDKN}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/fdkn_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/fdkn_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/fdkn_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/fdkn_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/fdkn_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/fdkn_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{PMBA}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/pmba_full_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/pmba_full_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/pmba_full_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/pmba_full_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/pmba_full_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/pmba_full_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{FDSR}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/FDSR_theirs_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/FDSR_theirs_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/FDSR_theirs_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/FDSR_theirs_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/FDSR_theirs_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/FDSR_theirs_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{Ours}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MID/ours_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/Middlebury/idx_\MIDbis/ours_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUv/ours_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/NYUv2/idx_\NYUvbis/ours_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLv/ours_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{diffs/DIML/idx_\DIMLvbis/ours_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{Ours Pred}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/ours_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/ours_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/ours_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/ours_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/ours_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/ours_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}
}
\caption{Qualitative comparison of upsampled depth maps. From top to bottom each group of two rows shows the error of upsampled images, defined as the difference between the prediction and the ground truth, on the Middlebury \cite{Scharstein2007,Scharstein2001,Scharstein2014,Scharstein2003,Hirschmuller2007}, NYUv2 \cite{Silberman2012} and DIML \cite{DIML1,DIML2,DIML3,DIML4} datasets, respectively; alternating between upsampling factors $\times8$ and $\times16$ for each dataset. From left to right, the first group of columns are (a) Guide, (b) Source and (c) Ground Truth; the second group includes selected methods from our quantitative evaluation, (d) SD filter \cite{Ham2018}, (e) Pixtransform \cite{deLutio2019}, (f) MSG-Net \cite{Tak-Wai2016}, (g) FDKN \cite{Kim2021}, (h) PMBANet \cite{Ye2020} and (i) FDSR \cite{he2021}; the last two columns represent (j) the error for the prediction of our model and (k) the prediction itself.}
\label{fig:depth_upsampling}
\vspace{-0.3cm}
\end{figure*}

==> tables/qualitative_results_v2.tex <==

%\newcommand\FigsGridWidth{0.106}
\newcommand\FigsGridWidth{0.09}
\newcommand\FigsGridVspace{0.05cm}
\newcommand\FigsGridVspacee{0.15cm}
\newcommand\FigsGridHspace{-0.22cm}
\newcommand\FigsGridHspacee{0.22cm}

\newcommand\MID{6}
\newcommand\MIDbis{400}

\newcommand\NYUv{5}
\newcommand\NYUvbis{3}

\newcommand\DIMLv{200}
\newcommand\DIMLvbis{1}


\begin{figure*}[t]
\vspace{-0.2cm}
  \centering
  \tiny	
% \begin{center}
% 	\hspace{1.5cm}\includegraphics[width=0.25\linewidth]{diffs/colorbar}\vspace{-.5cm}
% \end{center}

%0.141 0.106
\subfloat[{Guide.}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
        
        \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/guide_\MID.png}\vspace{\FigsGridVspace} 
        \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/guide_\MIDbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
        \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/guide_\NYUv.png}\vspace{\FigsGridVspace}
        \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/guide_\NYUvbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/guide_\DIMLv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/guide_\DIMLvbis.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{Source}.]{

    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/source_idx_\MID_scale_8.png}\vspace{\FigsGridVspace} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/source_idx_\MIDbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/source_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/source_idx_\NYUvbis_scale_16.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/source_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/source_idx_\DIMLvbis_scale_16.png}\vspace{\FigsGridVspace}
    \end{minipage}

}\hspace{\FigsGridHspace}
\subfloat[{GT}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/gt_idx_\MID.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/gt_idx_\MIDbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/gt_idx_\NYUv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/gt_idx_\NYUvbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/gt_idx_\DIMLv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/gt_idx_\DIMLvbis.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{SD}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/SDfilter_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/SDfilter_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/SDfilter_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/SDfilter_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/SDfilter_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/SDfilter_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{Pixtr}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/pixtransform_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/pixtransform_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}  
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/pixtransform_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/pixtransform_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/pixtransform_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/pixtransform_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{MSG}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/MSGNet_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/MSGNet_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/MSGNet_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/MSGNet_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/MSGNet_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/MSGNet_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{FDKN}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/fdkn_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/fdkn_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/fdkn_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/fdkn_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/fdkn_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/fdkn_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{PMBA}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/pmba_full_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/pmba_full_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/pmba_full_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/pmba_full_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/pmba_full_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/pmba_full_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{FDSR}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/FDSR_theirs_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/FDSR_theirs_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/FDSR_theirs_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/FDSR_theirs_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/FDSR_theirs_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/FDSR_theirs_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee} 
\subfloat[{LGR}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/_x8/LGR_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/LGR_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/LGR_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/LGR_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/LGR_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/LGR_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}
\subfloat[{DADA Pred}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/DADA_idx_\MID_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/DADA_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/DADA_idx_\NYUv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/DADA_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/DADA_idx_\DIMLv_scale_8.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/DADA_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}
\caption{Qualitative comparison of upsampled depth maps. From top to bottom each group of two rows shows the error of upsampled images, defined as the difference between the prediction and the ground truth, on the Middlebury \cite{Scharstein2007,Scharstein2001,Scharstein2014,Scharstein2003,Hirschmuller2007}, NYUv2 \cite{Silberman2012} and DIML \cite{DIML1,DIML2,DIML3,DIML4} datasets, respectively; alternating between upsampling factors $\times8$ and $\times16$ for each dataset. From left to right, the first group of columns are (a) Guide, (b) Source and (c) Ground Truth; the second group includes selected methods from our quantitative evaluation, (d) SD filter \cite{Ham2018}, (e) Pixtransform \cite{deLutio2019}, (f) MSG-Net \cite{Tak-Wai2016}, (g) FDKN \cite{Kim2021}, (h) PMBANet \cite{Ye2020} and (i) FDSR \cite{he2021}; the last two columns represent (j) the error for the prediction of our model and (k) the prediction itself.}
\label{fig:depth_upsampling}
\vspace{-0.3cm}
\end{figure*}

==> tables/qualitative_results_v3.tex <==

%\newcommand\FigsGridWidth{0.106}
\newcommand\FigsGridWidth{0.083}
\newcommand\FigsGridVspace{0.05cm}
\newcommand\FigsGridVspacee{0.15cm}
\newcommand\FigsGridHspace{-0.22cm}
\newcommand\FigsGridHspacee{0.22cm}

\newcommand\MID{6}
\newcommand\MIDbis{400}

\newcommand\NYUv{3}
\newcommand\NYUvbis{3}

\newcommand\DIMLv{200}
\newcommand\DIMLvbis{1}


\begin{figure*}[t]
\vspace{-0.2cm}
  \centering
  \tiny	
% \begin{center}
% 	\hspace{1.5cm}\includegraphics[width=0.25\linewidth]{diffs/colorbar}\vspace{-.5cm}
% \end{center}

%0.141 0.106
\subfloat[{Guide.}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
        
        \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/guide_\MID.png}\vspace{\FigsGridVspace} 
        \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/guide_\MIDbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
        \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/guide_\NYUv.png}\vspace{\FigsGridVspace}
        \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/guide_\NYUvbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/guide_\DIMLv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/guide_\DIMLvbis.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{Source}.]{

    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/source_idx_\MID_scale_16.png}\vspace{\FigsGridVspace} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/source_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/source_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/source_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/source_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/source_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}

}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{GT}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/gt_idx_\MID.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/gt_idx_\MIDbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/gt_idx_\NYUv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/gt_idx_\NYUvbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/gt_idx_\DIMLv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/gt_idx_\DIMLvbis.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{PixT}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/pixtransform_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/pixtransform_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}  
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/pixtransform_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/pixtransform_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/pixtransform_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/pixtransform_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{MSG}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/MSGNet_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/MSGNet_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/MSGNet_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/MSGNet_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/MSGNet_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/MSGNet_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{FDKN}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/fdkn_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/fdkn_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/fdkn_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/fdkn_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/fdkn_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/fdkn_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{PMBA}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/pmba_full_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/pmba_full_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/pmba_full_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/pmba_full_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/pmba_full_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/pmba_full_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{FDSR}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/FDSR_theirs_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/FDSR_theirs_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/FDSR_theirs_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/FDSR_theirs_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/FDSR_theirs_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/FDSR_theirs_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{LGR}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/LGR_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/LGR_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/LGR_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/LGR_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/LGR_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/LGR_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{DADA}.]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/DADA_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/DADA_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/DADA_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/DADA_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/DADA_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/DADA_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{DADA.}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/DADA_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/DADA_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/DADA_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/DADA_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/DADA_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/DADA_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}
\caption{ Results obtained by several of the considered methods. Rows from top to bottom: Middlebury $\times$16, Middlebury $\times$32, NYUv2 $\times$16, NYUv2 $\times$32, DIML $\times$16, DIML $\times$32. The residual images are displayed to highlight the errors' locations. All residual images in each row use the same color map. The last column shows the final results of our method.
% Qualitative comparison of upsampled depth maps. From top to bottom each group of two rows shows the error of upsampled images, defined as the difference between the prediction and the ground truth, on the Middlebury \cite{Scharstein2007,Scharstein2001,Scharstein2014,Scharstein2003,Hirschmuller2007}, NYUv2 \cite{Silberman2012} and DIML \cite{DIML1,DIML2,DIML3,DIML4} datasets, respectively; alternating between upsampling factors $\times8$ and $\times16$ for each dataset. From left to right, the first group of columns are (a) Guide, (b) Source and (c) Ground Truth; the second group includes selected methods from our quantitative evaluation, (d) SD filter \cite{Ham2018}, (e) Pixtransform \cite{deLutio2019}, (f) MSG-Net \cite{Tak-Wai2016}, (g) FDKN \cite{Kim2021}, (h) PMBANet \cite{Ye2020} and (i) FDSR \cite{he2021}; the last two columns represent (j) the error for the prediction of our model and (k) the prediction itself.
}
\label{fig:depth_upsampling}
\vspace{-0.3cm}
\end{figure*}

==> tables/qualitative_results_v4.tex <==

%\newcommand\FigsGridWidth{0.106}
\newcommand\FigsGridWidth{0.083}
\newcommand\FigsGridVspace{0.05cm}
\newcommand\FigsGridVspacee{0.15cm}
\newcommand\FigsGridHspace{-0.22cm}
\newcommand\FigsGridHspacee{0.22cm}

\newcommand\MID{6}
\newcommand\MIDbis{400}

\newcommand\NYUv{3}
\newcommand\NYUvbis{3}

\newcommand\DIMLv{200}
\newcommand\DIMLvbis{1}


\begin{figure*}[t]
\vspace{-0.2cm}
  \centering
  \tiny	
% \begin{center}
% 	\hspace{1.5cm}\includegraphics[width=0.25\linewidth]{diffs/colorbar}\vspace{-.5cm}
% \end{center}

%0.141 0.106
\subfloat[{Guide}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
        
        \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/guide_\MID.png}\vspace{\FigsGridVspace} 
        \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/guide_\MIDbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
        \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/guide_\NYUv.png}\vspace{\FigsGridVspace}
        \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/guide_\NYUvbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/guide_\DIMLv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/guide_\DIMLvbis.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{Source}]{

    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/source_idx_\MID_scale_16.png}\vspace{\FigsGridVspace} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/source_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/source_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/source_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/source_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/source_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}

}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{PixT}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/pixtransform_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/pixtransform_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}  
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/pixtransform_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/pixtransform_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/pixtransform_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/pixtransform_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{MSG}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/MSGNet_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/MSGNet_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/MSGNet_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/MSGNet_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/MSGNet_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/MSGNet_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{FDKN}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/fdkn_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/fdkn_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/fdkn_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/fdkn_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/fdkn_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/fdkn_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{PMBA}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/pmba_full_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/pmba_full_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/pmba_full_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/pmba_full_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/pmba_full_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/pmba_full_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{FDSR}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/FDSR_theirs_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/FDSR_theirs_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/FDSR_theirs_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/FDSR_theirs_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/FDSR_theirs_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/FDSR_theirs_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{LGR}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/LGR_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/LGR_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/LGR_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/LGR_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/LGR_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/LGR_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{DADA}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MID/DADA_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/Middlebury/idx_\MIDbis/DADA_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUv/DADA_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/NYUv2/idx_\NYUvbis/DADA_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLv/DADA_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{mydiffs/DIML/idx_\DIMLvbis/DADA_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{DADA}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/DADA_idx_\MID_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/DADA_idx_\MIDbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/DADA_idx_\NYUv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/DADA_idx_\NYUvbis_scale_32.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/DADA_idx_\DIMLv_scale_16.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/DADA_idx_\DIMLvbis_scale_32.png}\vspace{\FigsGridVspace}
    \end{minipage}
}\hspace{\FigsGridHspace}\hspace{\FigsGridHspacee}
\subfloat[{GT}]{
    \begin{minipage}[b]{\FigsGridWidth\linewidth} 
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MID/gt_idx_\MID.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/Middlebury/idx_\MIDbis/gt_idx_\MIDbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUv/gt_idx_\NYUv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/NYUv2/idx_\NYUvbis/gt_idx_\NYUvbis.png}\vspace{\FigsGridVspace}\vspace{\FigsGridVspacee}
    
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLv/gt_idx_\DIMLv.png}\vspace{\FigsGridVspace}
    \includegraphics[width=\linewidth]{images/DIML/idx_\DIMLvbis/gt_idx_\DIMLvbis.png}\vspace{\FigsGridVspace}
    \end{minipage}
}
\caption{Error maps for different guided super-resolution methods. Rows from top to bottom: Middlebury $\times$16, Middlebury $\times$32, NYUv2 $\times$16, NYUv2 $\times$32, DIML $\times$16, DIML $\times$32. Blue denotes under-estimated depth, red denotes over-estimation. All errors maps in a row have the same color scale. The last two columns juxtapose our predictions and the ground truth.
% Qualitative comparison of upsampled depth maps. From top to bottom each group of two rows shows the error of upsampled images, defined as the difference between the prediction and the ground truth, on the Middlebury \cite{Scharstein2007,Scharstein2001,Scharstein2014,Scharstein2003,Hirschmuller2007}, NYUv2 \cite{Silberman2012} and DIML \cite{DIML1,DIML2,DIML3,DIML4} datasets, respectively; alternating between upsampling factors $\times8$ and $\times16$ for each dataset. From left to right, the first group of columns are (a) Guide, (b) Source and (c) Ground Truth; the second group includes selected methods from our quantitative evaluation, (d) SD filter \cite{Ham2018}, (e) Pixtransform \cite{deLutio2019}, (f) MSG-Net \cite{Tak-Wai2016}, (g) FDKN \cite{Kim2021}, (h) PMBANet \cite{Ye2020} and (i) FDSR \cite{he2021}; the last two columns represent (j) the error for the prediction of our model and (k) the prediction itself.
}
\label{fig:depth_upsampling}
\vspace{-0.3cm}
\end{figure*}

==> tables/stability.tex <==
\begin{table}[h]
\centering
\footnotesize
\vspace{-0.2cm}
 \resizebox{0.45\textwidth}{!}{%
\begin{tabular}{l| cccc}
  \multicolumn{1}{c}{Scale} & x4 & x8 & x16 & x32 \\ \midrule 
 MSE $[$cm$^2]$       & 2.52$\pm$0.04 & 5.60$\pm$0.09 & 15.6$\pm$0.10   & 47.6$\pm$0.50  \\
 MAE $[$cm$]$         & 0.11$\pm$0.00 & 0.20$\pm$0.00 & 0.47$\pm$0.00  & 1.35$\pm$0.01 \\
 MAPE $[\%]$          & 0.04$\pm$0.00 & 0.07$\pm$0.00 & 0.17$\pm$0.00  & 0.46$\pm$0.00 \\
 VV $[\%]$            & 0.06$\pm$0.00 & 0.12$\pm$0.00 & 0.30$\pm$0.00  & 0.91$\pm$0.01 \\
 EE $[\%]$            & 0.82$\pm$0.02 & 1.43$\pm$0.01 & 2.92$\pm$0.02  & 8.09$\pm$0.03 \\
\end{tabular}%
 }%\usepackage{adjustbox}
\vspace{-0.1cm}
\caption{Variability of metrics, Middlebury dataset.}
\vspace{-0.1cm}
\label{tab:r5}
\end{table}

==> tables/table_ablations_v1.tex <==
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{l | cc}
        & MSE & MAE \\
        \midrule \midrule
        Base & 5.67 & 0.199 \\ %\midrule
        % \quad No up-/downsampling w/ U-Net &  5.92 & 0.215 \\
        \quad No ImageNet pretraining & 5.92 & 0.211 \\ %\midrule
        \quad Constant initialization of $\mathbf{Y}_0$  & 5.64 & 0.200 \\ 
        % \bottomrule
    \end{tabular}
    \caption{Influence of different design choices of our method on Middlebury $\times8$.}
    \label{tab:ablations}
\end{table}

==> tables/transfer_table_v1.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcc ccc cccc cc c}
 Testing Dataset & &  GF \cite{he2012guided} & SD filter \cite{ham2017robust} & Pixtransform \cite{lutio2019guided} & MSG-Net \cite{Tak-Wai2016} & FDKN \cite{Kim2021}  & PMBANet \cite{Ye2020} & FDSR \cite{he2021} & Graph - Colour & Graph & Ours\\ \hline \hline
 
 
\multirow{2}{*}{DIML}  & MSE & 34.1 &  44.9 & 23.0 & 5.76 & 6.74 & 7.35 & 7.73 & 20.5 & 4.95 & \textbf{4.58}\\ %\cline{2-11} 
                       & MAE  & 1.77 &  0.83 & 1.26 & 0.51 & 0.53 & 0.59 & 0.74 & 0.77 & 0.40 & \textbf{0.3813}\\
                       & MSE (low-resolution) & 17.7 & 1.45 & 6.19 & 6.16 & 0.20 & 0.04 & 0.45 & 0.03 & 0.002 & \textbf{0.0}
                       \\ \hline\hline

\multirow{2}{*}{Middlebury}  & MSE & 40.5  & 82.5 & 32.7 & 11.0 & 10.0 & 9.62 & 18.4 & 23.9 & 8.25 & \textbf{7.82}\\ %\cline{2-11} 
                             & MAE  & 1.49  & 0.86 & 0.82 & 0.54 & 0.43 & 0.46 & 0.73 & 0.91 & \textbf{0.35} & \textbf{0.35} \\
                             & MSE (low-resolution) & 17.9 & 1.86 &  22.5 & 5.01 & 0.20 & 0.06 & 7.20 & 0.08 & 0.001 & \textbf{0.0}
                             \\ \hline\hline

\end{tabular}%
}%\usepackage{adjustbox}
\caption{Performance comparison with the state-of-the-art algorithms on cross-dataset generalisation. All learned methods have been trained on the NYUv2 dataset \cite{Shelhamer2017}. The table shows the performance of the methods on the DIML \cite{DIML1,DIML2,DIML3,DIML4} and Middlebury \cite{Scharstein2007,Scharstein2001,Scharstein2014,Scharstein2003,Hirschmuller2007} datasets for a $\times 8$ upsampling factor. The table shows the MSE (in $\text{cm}^ 2$), MAE (in cm) and low-resolution MSE (in $\text{cm}^2$).
}
\label{tab:cmp_crosstesting}
\end{table*}

==> tables/transfer_table_v2.tex <==
\begin{table*}[t]
\centering
\small
% \resizebox{\textwidth}{!}{%
\begin{tabularx}{0.9\textwidth}{lc YYYYYY}
 Testing Dataset & Metric &  MSG-Net & FDKN   & PMBANet  & FDSR  & LGR & Ours\\ \hline \hline
 
 
\multirow{3}{*}{DIML}  & MSE & 5.76 & 6.74 & 7.35 & 7.73 &  4.95 & \textbf{4.58}\\ %\cline{2-11} 
                       & MAE  & 0.51 & 0.53 & 0.59 & 0.74 & 0.40 & \textbf{0.38}\\
                       & MSE (low-resolution) & 6.16 & 0.20 & 0.04 & 0.45 & 0.002 & \textbf{0.0}
                       \\ \midrule

\multirow{3}{*}{Middlebury}  & MSE &  11.0 & 10.0 & 9.62 & 18.4 &  8.25 & \textbf{7.82}\\ %\cline{2-11} 
                             & MAE  &  0.54 & 0.43 & 0.46 & 0.73 & \textbf{0.35} & \textbf{0.35} \\
                             & MSE (low-resolution) &  5.01 & 0.20 & 0.06 & 7.20 & 0.001 & \textbf{0.0}
                             \\ %\hline\hline

\end{tabularx}%
% }%\usepackage{adjustbox}
\caption{ross-dataset generalisation performance. All learned methods were trained on NYUv2, then tested on DIML and Middlebury, at upsampling factor $\times$8. Errors are $\text{cm}^ 2$ for the MSE and in com for the MAE. The MSE at low resolution,\ie, after downsampling the predicted target, indicates inconsistency with the forward model (linear downsampling).
}
\label{tab:cmp_crosstesting}
\end{table*}
